Convergence of Invariant Graph Networks

Although theoretical properties such as expressive power and over-smoothing of graph neural networks (GNN) have been extensively studied recently, its convergence property is a relatively new direction. In this paper, we investigate the convergence of one powerful GNN, Invariant Graph Network (IGN) over graphs sampled from graphons. We first prove the stability of linear layers for general $k$-IGN (of order $k$) based on a novel interpretation of linear equivariant layers. Building upon this result, we prove the convergence of $k$-IGN under the model of \citet{ruiz2020graphon}, where we access the edge weight but the convergence error is measured for graphon inputs. Under the more natural (and more challenging) setting of \citet{keriven2020convergence} where one can only access 0-1 adjacency matrix sampled according to edge probability, we first show a negative result that the convergence of any IGN is not possible. We then obtain the convergence of a subset of IGNs, denoted as IGN-small, after the edge probability estimation. We show that IGN-small still contains function class rich enough that can approximate spectral GNNs arbitrarily well. Lastly, we perform experiments on various graphon models to verify our statements.

==> newproof.tex <==
\convergenceafterEM*

\begin{proof}
Using the triangle inequality
\begin{align*}
& MSE_U(\Phi_c(W), \Phi_d(\hat{W})) \\
& = \|S_U \Phi_c(W)-\frac{1}{n}\Phi_d (\hat{W}) \| \\ 
& = \|S_U \Phi_c(W)- S_U\Phi_c(\inducedW) + S_U\Phi_c(\inducedW) - \Phi_dS_U(\inducedW) + \Phi_dS_U(\inducedW) - \frac{1}{n}\Phi_d (\hat{W})\|\\
&\leq \underbrace{\|S_U \Phi_c(W)- S_U\Phi_c(\inducedW)\|}_\text{First term: discrization error} + 
\underbrace{\|S_U\Phi_c(\inducedW) - \Phi_dS_U(\inducedW)\|}_\text{Second term: sampling error} + \underbrace{\|\Phi_dS_U(\inducedW) - \frac{1}{n}\Phi_d (\hat{W})\|}_\text{Third term: estimation error} \numberthis \label{equ:threeterms} %
\end{align*}
The three terms measures the different sources of error. First term is concerned with the discreization error. Second term concerns the sampling error from randomness of $U$. This term will vanish if we consider only $S_n$ instead of $S_U$.
The third term concerns the edge probablity estimation error.

For the first term $\|S_U \Phi_c(W) - S_U \Phi_c (\inducedW) \| = \| S_U(\Phi_c(W) - \Phi_c(\inducedW))\|$, if suffices to upper bound $\|\Phi_c(W)-\Phi_c(\inducedW)\|_{L_\infty}$ according to property of $S_U$. Since $\| \Phi_c W - \Phi_c \inducedW\|_{L_\infty} \leq C\|W - \inducedW\|_{L_\infty}$ by \Cref{corollary:$k$-IGN-convergence}, and $\|W - \inducedW\|_{L_\infty}$ converges to 0 in probability according to \Cref{lem:inducedW-converges}, we conclude that the first term will converges to 0 with high probability. 


For the third term $\| \Phi_d S_U (\inducedW) - \frac{1}{n}\Phi_d (\hat{W})\| = \| \Phi_d S_U (\inducedW) - \Phi_d (\frac{1}{n}\hat{W})\| $, we know that $\|S_U(\inducedW) -  \frac{1}{n}\hat{W}\|_2 = \frac{1}{n}\|\hat{W}_{n\times n} - W_{n\times n}\|_2 \leq \|\hat{W}_{n\times n} - W_{n\times n}\|_{2, \infty}$, which will also goes to 0 with high probability as $n$ increases according to the statistical guarantee of edge probability estimation of neighborhood smoothing algorithm \citep{zhang2015estimating}, stated in \Cref{thm:graphon-estimation}. Therefore by \Cref{corollary:$k$-IGN-convergence}, the last term also goes to 0 with high probability.   

Therefore the rest work is to control the second term $\|S_U \Phi_c(\inducedW) - \Phi_d S_U(\inducedW)\|$. Again, we use the triangle inequality
\begin{align*}
& \tn{Second term} \\
& = \|S_U \Phi_c(\inducedW) - \Phi_d S_U(\inducedW)\| \\
& \leq \|S_U \Phi_c(\inducedW) - \sampleE \Phi_c(\inducedEW) \| + \| \sampleE \Phi_c(\inducedEW) - \Phi_d S_U(\inducedW)\| \\
& =  \|S_U \Phi_c(\inducedW) - \sampleE \Phi_c(\inducedEW) \| + \| \sampleE \Phi_c(\inducedEW) - \Phi_d \sampleE(\inducedEW)\|\\
& = \|S_U \Phi_c(\inducedW) - \sampleE \Phi_c(\inducedEW) \|\\
& \leq \|S_U \Phi_c(\inducedW) - S_U \Phi_c(\inducedEW)\| + \|S_U \Phi_c(\inducedEW) - \sampleE \Phi_c(\inducedEW)  \| \\
& = \underbrace{\|S_U (\Phi_c \inducedW - \Phi_c \inducedEW)\|}_\text{term $a$} + 
\underbrace{\|(S_U - \sampleE)\Phi_c(\inducedEW) \|}_\text{term $b$}
\end{align*}
The second equality holds because $S_U(\inducedW) = S_n(\inducedEW)$ by definition of $\inducedEW$. The third equality holds because for $\inducedEW$, evaluation operator $S_n$ and linear permutation equivariant $\Phi$ commutes according to \Cref{lem:T-shrinks-L-inf-norm}. 
We will bound the term a) $\|S_U (\Phi_c \inducedW - \Phi_c \inducedEW)\|$ and b) $\|(S_U - \sampleE)\Phi_c(\inducedEW) \|$ next. 

For term a) $\|S_U (\Phi_c \inducedW - \Phi_c \inducedEW)\|$, if suffices to prove that $\|\Phi_c \inducedW -\Phi_c \inducedEW)\|_{L_\infty}$ converges to 0 with high probability. Since $\|\Phi_c \inducedW - \Phi_c \inducedEW)\|_{L_\infty} \leq C\|\inducedW - \inducedEW \|_{L_\infty} \leq C(\|\inducedW - W \|_{L_\infty} + \|\inducedEW - W \|_{L_\infty})$, we only need to upper bound $\|\inducedW - W \|_{L_\infty}$ and $\|\inducedEW - W \|_{L_\infty}$, which are proved by \Cref{lem:inducedW-converges} and \Cref{lem:inducedEW-converges} respectively. 


For term b) $\|(S_U - \sampleE)\Phi_c(\inducedEW) \|$
\begin{align*}
&\|(S_U - \sampleE)\Phi_c(\inducedEW) \| \\
&= \|(S_U \Phi_c(\inducedEW) - \sampleE \Phi_c(\inducedEW)\|\\
& = \|(S_U \Phi_c(\inducedEW) - S_U \Phi_c(W) + S_U \Phi_c(W) - S_n \Phi_c(W) + S_n \Phi_c(W) - \sampleE \Phi_c(\inducedEW)\| \\
& \leq \|(S_U \Phi_c(\inducedEW) - S_U \Phi_c(W) \| + \|S_U \Phi_c(W) - S_n \Phi_c(W)\|  + \|S_n \Phi_c(W) - \sampleE \Phi_c(\inducedEW)\|\\
& \leq \|(S_U (\Phi_c\inducedEW-\Phi_c W) \| + \|S_U \Phi_c(W) - S_n \Phi_c(W)\| + \|\sampleE (\Phi_c\inducedEW-\Phi_c W)\|
\end{align*}
For the first and last term, by the property of $S_U, S_n$ and $\Phi_c$, it suffices to bound $\|W-\inducedEW \|_{L_\infty}$. As $\|W-\inducedEW \|_{L_\infty}$ converges to 0 almost surely (therefore in probablity) by \Cref{lem:inducedEW-converges}, we conclude that the first and last term converges to 0 almost surely. 
For the second term $\|S_U \Phi_c(W) - S_n \Phi_c(W)\|$, it converges to 0 almost surely according to the second part of \Cref{lem:sxsn-sampling}. 



As all terms converge to 0 in the probability or almost surely, we conclude that $\|S_U \Phi_c(W)-\Phi_d (\hat{W}) \|$ converges to 0 in probability.
\end{proof}


==> oldproof.tex <==
\begin{proof}
Using the triangle inequality
\begin{align*}
& MSE_U(T_c(W), T_d(\hat{W})) \\
& = \|S_U T_c(W)-\frac{1}{n}T_d (\hat{W}) \| \\ 
& = \|S_U T_c(W)- S_UT_c(\inducedW) + S_UT_c(\inducedW) - T_dS_U(\inducedW) + T_dS_U(\inducedW) - \frac{1}{n}T_d (\hat{W})\|\\
&\leq \underbrace{\|S_U T_c(W)- S_UT_c(\inducedW)\|}_\text{First term} + 
\underbrace{\|S_UT_c(\inducedW) - T_dS_U(\inducedW)\|}_\text{Second term} + \underbrace{\|T_dS_U(\inducedW) - \frac{1}{n}T_d (\hat{W})\|}_\text{Third term} %
\end{align*}
The three terms measures the different sources of error. First term is concerned with the discreization error. Second term concerns the sampling error from randomness of $U$. This term will vanish if we consider only $S_n$ instead of $S_U$.
The third term concerns the edge probablity estimation error.

For the first term $\|S_U T_c(W) - S_U T_c (\inducedW) \| = \| S_U(T_c(W) - T_c(\inducedW))\|$, if suffices to upper bound $\|T_c(W)-T_c(\inducedW)\|_{L_\infty}$ according to property of $S_U$. Since $\| T_c (W - \inducedW)\|_{L_\infty} \leq C\|W - \inducedW\|_{L_\infty}$ by \Cref{corollary:$k$-IGN-convergence}, and $\|W - \inducedW\|_{L_\infty}$ converges to 0 in probability according to \Cref{lem:inducedW-converges}, we conclude that the first term will converges to 0 with high probability. Note that \Cref{lem:inducedW-converges} relies on $W$ beling \lip{} and will not hold in later layers. 

\textcolor{blue}{For the first term $\|S_U T_c(W) - S_U T_c (\inducedW) \| = \| S_U(T_c(W) - T_c(\inducedW))\|$, if suffices to upper bound $\|T_c(W)-T_c(\inducedW)\|_{L_2}$ according to NEW property of $S_U$. Since $\| T_c (W - \inducedW)\|_{L_2} \leq C\|W - \inducedW\|_{L_2}$ by \Cref{thm:$2$-IGN-convergence}, and $\|W - \inducedW\|_{L_2}$ converges to 0 in probability according to second part of \Cref{lem:inducedW-converges}. Therefore we conclude that the first term will converges to 0 with high probability. 
}


For the third term $\| T_d S_U (\inducedW) - \frac{1}{n}T_d (\hat{W})\|$, we know that $\|S_U(\inducedW) -  \frac{1}{n}\hat{W}\|_2 = \frac{1}{n}\|\hat{W}_{n\times n} - W_{n\times n}\|_2 \leq \|\hat{W}_{n\times n} - W_{n\times n}\|_{2, \infty}$, which will also goes to 0 with high probability as $n$ increases according to the statistical guarantee of edge probability estimation of neighborhood smoothing algorithm \citep{zhang2015estimating}, stated in \Cref{thm:graphon-estimation}. Therefore by \Cref{corollary:$k$-IGN-convergence}, the last term also goes to 0 with high probability.   

Therefore the rest work is to control the second term $\|S_U T_c(\inducedW) - T_d S_U(\inducedW)\|$. Again, we use the triangle inequality
\begin{align*}
& \tn{Second term} \\
& = \|S_U T_c(\inducedW) - T_d S_U(\inducedW)\| \\
& \leq \|S_U T_c(\inducedW) - \sampleE T_c(\inducedEW) \| + \| \sampleE T_c(\inducedEW) - T_d S_U(\inducedW)\| \\
& =  \|S_U T_c(\inducedW) - \sampleE T_c(\inducedEW) \| + \| \sampleE T_c(\inducedEW) - T_d \sampleE(\inducedEW)\|\\
& = \|S_U T_c(\inducedW) - \sampleE T_c(\inducedEW) \|\\
& \leq \|S_U T_c(\inducedW) - S_U T_c(\inducedEW)\| + \|S_U T_c(\inducedEW) - \sampleE T_c(\inducedEW)  \| \\
& = \underbrace{\|S_U T_c (\inducedW - \inducedEW)\|}_\text{term $a$} + 
\underbrace{\|(S_U - \sampleE)T_c(\inducedEW) \|}_\text{term $b$}
\end{align*}
The second equality holds because $S_U(\inducedW) = S_n(\inducedEW)$. The third equality holds because for $\inducedEW$, evaluation operator $S_n$ and linear permutation equivariant $T$ commutes. 
We will bound the term a) $\|S_U T_c (\inducedW - \inducedEW)\|$ and b) $\|(S_U - \sampleE)T_c(\inducedEW) \|$ next. 

For term a) $\|S_U T_c (\inducedW - \inducedEW)\|$, if suffices to prove that $\|T_c (\inducedW - \inducedEW)\|_{L_\infty}$ converges to 0 with high probability. Since $\|T_c (\inducedW - \inducedEW)\|_{L_\infty} \leq C\|\inducedW - \inducedEW \|_{L_\infty} \leq C|\|\inducedW - W \|_{L_\infty} + \|\inducedEW - W \|_{L_\infty}|$, we only need to bound $\|\inducedW - W \|_{L_\infty}$ and $\|\inducedEW - W \|_{L_\infty}$, which are proved by \Cref{lem:inducedW-converges} and \Cref{lem:inducedEW-converges} respectively. %

\textcolor{blue}{For term a) $\|S_U T_c (\inducedW - \inducedEW)\|$, if suffices to prove that $\|T_c (\inducedW - \inducedEW)\|_{L_2}$ converges to 0 with high probability. Since $\|T_c (\inducedW - \inducedEW)\|_{L_2} \leq C\|\inducedW - \inducedEW \|_{L_2} \leq C|\|\inducedW - W \|_{L_2} + \|\inducedEW - W \|_{L_2}|$, we only need to bound $\|\inducedW - W \|_{L_2}$ and $\|\inducedEW - W \|_{L_2}$, which are proved by \Cref{lem:inducedW-converges} and \Cref{lem:inducedEW-converges} respectively.}


For term b) $\|(S_U - \sampleE)T_c(\inducedEW) \|$
\begin{align*}
&\|(S_U - \sampleE)T_c(\inducedEW) \| \\
&= \|(S_U T_c(\inducedEW) - \sampleE T_c(\inducedEW)\|\\
& = \|(S_U T_c(\inducedEW) - S_U T_c(W) + S_U T_c(W) - S_n T_c(W) + S_n T_c(W) - \sampleE T_c(\inducedEW)\| \\
& \leq \|(S_U T_c(\inducedEW) - S_U T_c(W) \| + \|S_U T_c(W) - S_n T_c(W)\|  + \|S_n T_c(W) - \sampleE T_c(\inducedEW)\|\\
& \leq \|(S_U T_c(\inducedEW-W) \| + \|S_U T_c(W) - S_n T_c(W)\| + \|\sampleE T_c(\inducedEW-W)\|
\end{align*}
For the first and last term, by the property of $S_U, S_n$ and $T_c$, it suffices to bound $\|W-\inducedEW \|_{L_\infty}$. As $\|W-\inducedEW \|_{L_\infty}$ converges to 0 almost surely by \Cref{lem:inducedEW-converges}, we conclude that the first and last term converges to 0 almost surely. 
For the second term $\|S_U T_c(W) - S_n T_c(W)\|$, it converges to 0 almost surely according to second part of \Cref{lem:sxsn-sampling}. 


\textcolor{blue}{For the first and last term, by the property of $S_U, S_n$ and $T_c$, if suffices to bound $\|W-\inducedEW \|_{L_2}$. As $\|W-\inducedEW \|_{L_2}$ converges to 0 almost surely by \Cref{lem:inducedEW-converges}, we conclude that first and last term converges to 0 almost surely. 
For the second term $\|S_U T_c(W) - S_n T_c(W)\|$, it converges to 0 almost surely according to second part of \Cref{lem:sxsn-sampling}.}


As all terms converge to 0 in the probability or almost surely, we conclude that $\|S_U T_c(W)-T_d (\hat{W}) \|$ converges to 0 in probability.
\end{proof}

